WINGS: Reference-Free Gaussian Splatting Inpainting with 3D-Native Generative Priors

Inpainting 3D Gaussian Splatting scenes, a key challenge in 3D editing, requires generating plausible content within a masked region of 3D space. Prior approaches rely on 2D diffusion models to produce one or several inpainted reference views, making them susceptible to challenges associated with multi-view inconsistency and lengthy optimization times. Departing from these approaches, we introduce a reference-free Gaussian splatting inpainting method operating natively in 3D. Our method leverages the embedding space of a large, pre-trained 3D prior, combined with a structure completion network to feed a generative prior which reconstructs the missing region's geometry and appearance. Performing content generation entirely in 3D, it avoids the need to reconcile inconsistencies of multiple inpainted reference images, and is faster than related 2D-based methods. We demonstrate the effectiveness of our method qualitatively and quantitatively, through extensive experiments and a user study. To the best of our knowledge, this work is the first Gaussian splatting inpainting method to operate in the learned representation space of a 3D-native generative prior without relying on inpainted reference views.

==> latexmkrc <==
#!/usr/bin/perl

#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}



## Put this (Perl) file in the root of your Overleaf project. It overrides the
## `pdflatex` compilation command to run GhostScript as a post-process which will
## compress non-JPEG images to JPEG in the output PDF file. The JPEG quality
## settings are set to high to minimize the loss of image quality. This should
## work well even for images that contain a lot of high-frequency noise.
## To disable, simply rename the file to something other than latexmkrc.
##
## Created by Iliyan Georgiev.

## Quality settings
$PDF_VERSION = 1.4;
$IMG_DOWNSAMPLE = 'true';
$IMG_DOWNSAMPLE_DPI = 600;
$IMG_DOWNSAMPLE_THRESHOLD = 1.0;
$IMG_COMPRESSION_QFACTOR = 0.2;  # lower is better (try 0.08 for higher quality)
$PASSTHROUGH_JPEGS = 'true';

## Don't modify these, they are specified by Overleaf
$GS_INPUT_FILE = '%B.pdf';
$GS_OUTPUT_FILE = '%B-embed.pdf';

## You can try setting below: -dNEWPDF=true
## This fails in the current GhostScript v9.55 on Overleaf 
$GS_COMMAND = "gs
   -sDEVICE=pdfwrite
   -sOutputFile=$GS_OUTPUT_FILE
   -dCompatibilityLevel=$PDF_VERSION
   -dPDFSETTINGS=/default
   -dFastWebView=true
   -dEmbedAllFonts=true
   -dSubsetFonts=true
   -dCompressFonts=true
   -dDetectDuplicateImages=true
   -dDoThumbnails=false
   -dAutoRotatePages=/None
   -dDownsampleColorImages=$IMG_DOWNSAMPLE
   -dColorImageDownsampleType=/Bicubic
   -dColorImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dColorImageResolution=$IMG_DOWNSAMPLE_DPI
   -dDownsampleGrayImages=$IMG_DOWNSAMPLE
   -dGrayImageDownsampleType=/Bicubic
   -dGrayImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dGrayImageResolution=$IMG_DOWNSAMPLE_DPI
   -dDownsampleMonoImages=$IMG_DOWNSAMPLE
   -dMonoImageDownsampleType=/Subsample
   -dMonoImageDownsampleThreshold=$IMG_DOWNSAMPLE_THRESHOLD
   -dMonoImageResolution=$IMG_DOWNSAMPLE_DPI
   -dConvertCMYKImagesToRGB=true
   -dColorImageFilter=/DCTEncode
   -dGrayImageFilter=/DCTEncode
   -dMonoImageFilter=/CCITTFaxEncode
   -dColorConversionStrategy=/LeaveColorUnchanged
   -dPassThroughJPEGImages=$PASSTHROUGH_JPEGS
   -dProcessColorModel=/DeviceRGB
   -dRenderIntent=1
   -dDefaultRenderingIntent=/Perceptual
   -dUseArtBox
   -dNEWPDF=false
   -dNOPAUSE
   -dBATCH
   -c \"<< /ColorACSImageDict << /VSamples [ 1 1 1 1 ] /HSamples [ 1 1 1 1 ] /QFactor $IMG_COMPRESSION_QFACTOR /Blend 1 /ColorTransform 1 >> >> setdistillerparams\"
   -f $GS_INPUT_FILE";

## Remove new-line characters from GhostScript command
$GS_COMMAND =~ s/\n//g;

## Set the pdflatex command to be used by Overleaf
$pdflatex = "pdflatex %O %S; $GS_COMMAND; mv %B-embed.pdf %B.pdf";

## For debugging
# print "$GS_COMMAND\n";
# print "$pdflatex\n";



==> storage.tex <==
# Intro

\MF{method paragraph; currently undercomplex and badly worded. needs refinement.} Given a masked region where an object has been removed and a 3DGS scene, we embed them into TRELLIS' structured latent embedding.
We mask the SLAT latents. 
TRELLIS is very general, but has a TRELLIS-specific look (plasticy) \EM{TRELLIS is also very asset-oriented, as opposed to the scene-level 3DGS data we apply it on}. We do not want to discard its learned prior, as well as can not afford to train the whole model, so we adapt it to our scene's specific appearance via a per-scene LoRA. \MF{conflates geometry and appearance}
Doing so allows us to efficiently sample from a conditional distribution using the general prior.
We need to reconstruct the masked SLAT's, to do so we use a pre-trained structure completion network that purely predicts occupancy. 
Subsequently, we need to generate features for the newly created, occupancy-only SLATs that align with the surrounding context region, so that the decoder can blend them seamlessly into the scene. 
We use TRELLIS' Flow Matching model \EM{with our own attention scheduling} for this and generate \acp{SLAT} that are consistent with the scene's appearance and seamlessly blend back into the original scene after decoding. 

Importantly, our approach pays explicit attention to the masked region's \emph{context}, i.e., the visual statistics of the surrounding area, to create an artifact-free and seamlessly blending inpainting results. 
\MF{TODO: refine approach description}


Our approach requires no reference views inpainted by a 2D model: hence, it is multiview-consistent by design. Moreover, our proposed approach runs in a single network execution and requires no post-optimization of the existing scene, making it fast and allowing to inpaint a scene in few (1-3) minutes. 
It further explicitly takes scene context into account to generate seamless Gaussians.

These characteristics are crucial for promoting interactive 3D Gaussian splatting with users, enabling downstream creative and (?) applications.
In summary, our contributions are \MF{TODO, rework or refine}: 

\begin{itemize}
    \item We introduce a novel pipeline for inpainting \ac{3DGS} scenes by leveraging a 3D-native prior. Contrary to previous approaches, we do not rely on reference views inpainted by a 2D model and instead use a 3D-native generative model that is multi-view consistent by construction.
    \item We also introduce a mechanism to efficiently sample from a conditional distribution using the general prior. \EM{adaptation of 3D sampling to context}
    \item We introduce a mechanism that adapts the scene specific Gaussian primitive distribution large-scale pre-trained generative priors to scene-specific distributions of Gaussians. \EM{too generic}
\end{itemize}

\EM{Should we use the term "test-time training" to describe the fact that we train a LoRA on the fly, that it is optional but really improves results?}

Our approach is substantially faster than related 2D methods and provides on-par or higher quality. 
We prove the effectiveness of our method through quantitiative and qualitiative experiments and a user study, and see this work as a first step towards 3D-native content editing. 

\section{appendix}


\subsection{Relationship with 3DGS-MCMC}

\paragraph{Probability density of Gaussians in a scene}

\NL{I'm putting this section in the supplementary in case we want to keep it. The posterior formulation was written with DPS in mind, because then the likelihood $\mathcal{P}(I | G_m, G_c)$ is not inactive, making the bayesian factorisation very relevant. In the current state of the paper, we are not doing DPS and thus the framework becomes less motivated. The conditional prior is probably suficient.}

In this work, we leverage a Bayesian interpretation \MF{why? lacks motivation} of the 3DGS-MCMC formalization introduced by~\cite{kheradmand_3d_2025} and define a data-dependent probability density $\mathcal{P}$ over Gaussian configurations \MF{consistent with images $I$}:  
\begin{equation}\label{eq:3dgs-mcmc}
   \mathcal{P}(G) \propto \exp \left( -\mathcal{L}_{total}(G; I) \right), \, \text{where}
\end{equation}
$$\mathcal{L}_{total}(G; I) = (1 - \lambda_{\text{DSSIM}}) \cdot \mathcal{L}_1 + \lambda_{\text{DSSIM}} \cdot \mathcal{L}_{\text{DSSIM}} + \lambda_o \cdot \sum_i |o_i| + \lambda_\Sigma  \sum_{ij} \left|\sqrt{\text{eig}_j(\Sigma_i)} \right|_1.$$
\MF{$o$ not introduced, e.g. $o_i$ and $\lambda_o$, same for $\Sigma$}The density probability $\mathcal{P}(G)$ implicitely depends on the training observations through the reconstruction loss; here, we make this dependence explicit and write $\mathcal{P}(G | I)$.
Noticing that only $\mathcal{L}_1$ and $\mathcal{L}_{\text{DSSIM}}$ are data-dependent, we decompose $\mathcal{L}_{total}(G; I) = \mathcal{L}_{data}(G; I) + \mathcal{L}_{reg}(G)$ 
%the sum of respectively a data-dependent loss and a regularization loss. 
and rewrite \Cref{eq:3dgs-mcmc} as $$\mathcal{P}(G) \propto \exp \left( -\mathcal{L}_{data} \right) \cdot \exp \left( -\mathcal{L}_{reg} \right).$$ 
By identification, we define the data-dependent likelihood and a prior over the distribution of Gaussians:
\begin{equation}
    \begin{aligned}
        \mathcal{P}(I | G) & \propto \exp ( - \mathcal{L}_{data}(G; I)) \\
         \tilde{\mathcal{P}}(G) & \propto \exp (- \mathcal{L}_{reg}(G))
    \end{aligned}
\end{equation}
The probability density of Gaussians in \Cref{eq:3dgs-mcmc} can therefore be viewed as a posterior distribution, yielding the following factorization through Bayes' rule:
\begin{equation}\label{eq:3dgs-mcmc-bayes}
    \mathcal{P}(G | I) \propto \mathcal{P}(I | G) \cdot \tilde{\mathcal{P}}(G)
\end{equation}

 \paragraph{Inpainting}

Inpainting a 3DGS scene requires generating plausible content in a masked region based on surrounding context-Gaussians. 
Let $G = G_m \cup G_c$, where $G_m$ are Gaussians masked by a binary mask $M$, i.e. the region to inpaint, and $G_c$ represents context information.
Sampling masked region Gaussians from $\mathcal{P}(G|I)$ is thus equivalent to sampling from the conditional distribution:
$$
\mathcal{P}(G_m | G_c, I_c)
$$
where $I_c = I \odot (1 -\mathcal{R}(M))$ and $\mathcal{R}$ is the projection of the 3D mask to pixel space. Using the same Bayes factorization as (\ref{eq:3dgs-mcmc-bayes}) yields:
\begin{equation} \label{eq:inpainting-problem}
\begin{aligned}
    \mathcal{P}(G_m | G_c, I_c) & \propto \mathcal{P}(I_c | G_m, G_c) \cdot \tilde{\mathcal{P}}(G_m | G_c) 
\end{aligned}
\end{equation}
    % & \propto \mathcal{P}(I_c | G_m, G_c) \cdot \frac{\tilde{\mathcal{P}}(G_m, G_c)}{\tilde{\mathcal{P}}(G_c)} \\
    % & \propto \mathcal{P}(I_c | G_m, G_c) \cdot \tilde{\mathcal{P}}(G) \\
%since $\tilde{\mathcal{P}}(G)$ is constant with respect to $G_m$. 
Because the masked region is by definition unobserved, generation of masked Gaussians needs to rely on the conditional prior rather than the image likelihood. However, the regularization prior $\tilde{\mathcal{P}}(G)$ of~\cite{kheradmand_3d_2025} is only designed to constrain the opacity and size of the Gaussians during optimization with respect to observed images, and thus provides no representation of scene geometry and appearance in an unobserved region. In this work, we propose to replace it with a learned generative prior $\mathcal{P}_\theta(G)$ to generate Gaussians in the masked region. 

\MF{the entire above section needs to be better motivated and connected to the actual pipeline.}
